Addressing Gap between Training Data and Deployed Environment by On-Device Learning

The accuracy of tinyML applications is often affected by various environmental factors, such as noises, location/calibration of sensors, and time-related changes. This article introduces a neural network based on-device learning (ODL) approach to address this issue by retraining in deployed environments. Our approach relies on semi-supervised sequential training of multiple neural networks tailored for low-end edge devices. This article introduces its algorithm and implementation on wireless sensor nodes consisting of a Raspberry Pi Pico and low-power wireless module. Experiments using vibration patterns of rotating machines demonstrate that retraining by ODL improves anomaly detection accuracy compared with a prediction-only deep neural network in a noisy environment. The results also show that the ODL approach can save communication cost and energy consumption for battery-powered Internet of Things devices.

==> Makefile <==
LATEX   = platex
BIBTEX  = pbibtex
DVIPS   = dvips
DVIPDF  = dvipdfmx
TARGET  = main
TEXFILE = $(TARGET).tex	\
	refer.bib

all: $(TARGET).dvi

dvi: $(TARGET).dvi
$(TARGET).dvi: $(TEXFILE)
	$(LATEX) $(TARGET)
#	$(BIBTEX) $(TARGET)
#	$(LATEX) $(TARGET)
	$(LATEX) $(TARGET)

ps: $(TARGET).ps
$(TARGET).ps: $(TARGET).dvi
	$(DVIPS) -f $(TARGET).dvi > $(TARGET).ps

pdf: $(TARGET).pdf
$(TARGET).pdf: $(TARGET).dvi
	$(DVIPDF) $(TARGET).dvi

clean:
	rm -f $(TARGET).dvi
	rm -f $(TARGET).ps
	rm -f $(TARGET).log
	rm -f $(TARGET).out
	rm -f $(TARGET).pdf
	#rm -f $(TARGET).bbl
	rm -f $(TARGET).blg
	rm -f *.aux *~ 

